Demystifying Reachability in Vector Addition Systems

More than 30 years after their inception, the decidability proofs for reachability in vector addition systems (VAS) still retain much of their mystery. These proofs rely crucially on a decomposition of runs successively refined by Mayr, Kosaraju, and Lambert, which appears rather magical, and for which no complexity upper bound is known. We first offer a justification for this decomposition technique, by showing that it computes the ideal decomposition of the set of runs, using the natural embedding relation between runs as well quasi ordering. In a second part, we apply recent results on the complexity of termination thanks to well quasi orders and well orders to obtain a cubic Ackermann upper bound for the decomposition algorithms, thus providing the first known upper bounds for general VAS reachability.

==> proof-cartesian.tex <==
\begin{proof}
  First of all, let us prove that $I=I_1\times I_2$ is an ideal of
  $\ideal{S}{\preceq}$ for every $I_1\in \ideal{S_1}{\preceq_1}$ and
  $I_2\in\ideal{S_2}{\preceq_2}$. Let us consider $x,y\in I$. These
  elements can be decomposed into $x=(x_1,x_2)$ and $y=(y_1,y_2)$
  where $x_1,y_1\in I_1$ and $x_2,y_2\in I_2$. Since $I_1$ and $I_2$
  are ideals, there exists $m_1\in I_1$ and $m_2\in I_2$ such that
  $x_1\preceq_1 m_1$, $y_1\preceq_1 m_1$, $x_2\preceq_2 m_2$ and
  $y_2\preceq_2 m_2$. Let $m=(m_1,m_2)$ and observe that $m\in I$,
  $x\preceq m$, and $y\preceq m$. Thus $I$ is an ideal.
  
  Conversely, let us consider an ideal $I$ of $(S,\preceq)$. The
  projections $I_1=\bigcup_{x_2\in S_2}\{s_1\in S_1\mid (s_1,x_2)\in
  I\}$ and $I_2=\bigcup_{x_1\in S_1}\{s_2\in S_2\mid (x_1,s_2)\in I\}$
  are clearly ideals, moreover $I\subseteq I_1\times I_2$. Conversely,
  let us consider $s_1\in I_1$ and $s_2\in I_2$ and let us prove that
  $(s_1,s_2)\in I$. There exists $x_2\in S_2$ such that $(s_1,x_2)\in
  I$ and $x_1\in S_1$ such that $(x_1,s_2)\in I$. As $I$ is an ideal,
  there exists $(m_1,m_2)\in I$ such that $(s_1,x_2),(x_1,s_2)\preceq
  (m_1,m_2)$. Hence $(s_1,s_2)\preceq (m_1,m_2)$. As $I$ is downward
  closed, we deduce that $(s_1,s_2)\in I$. We have proved the other
  inclusion $I_1\times I_2\subseteq I$.
\end{proof}
%

==> proof-connected.tex <==
\begin{proof}
  Let us write ${\downarrow}\runs=J\cup J_1\cup\cdots\cup J_k$ for the
  canonical decomposition of ${\downarrow}\runs$.  By minimality of
  this decomposition, there is a prerun $\rho$ in $J$ such that
  $\rho\not\in J_j$ for any $1\leq j\leq k$.  Thus any run in
  ${\uparrow}\rho\cap\runs$ must belong to~$J$.

  By \autoref{lem:limit}, $J=\lim_n\rho_n$ for a non-decreasing
  sequence of preruns $(\rho_n)_n$.  We build inductively a new
  sequence $(\rho'_n)_n$ of \emph{runs} in $J$ such that
  $\rho\unlhd\rho'_n$ and $\rho_n\unlhd\rho'_n$ for all $n$; this will
  entail $J=\lim_n\rho'_n$.  Initially, because $J$ is directed there
  exists a prerun $\rho'$ such that $\rho,\rho_0\unlhd\rho'$.  Since
  $J\subseteq{\downarrow}\runs$, there exists a run $\rho'_0$ such
  that $\rho'\unlhd\rho'_0$.  Because $\rho\unlhd\rho'_0$ and by the
  remark made in the first paragraph of this proof, this run
  belongs to $J$.  For the induction step, we apply the same reasoning
  to a prerun $\rho'$ in $J$ with $\rho_n,\rho'_n\unlhd\rho'$ to build
  the run~$\rho'_{n+1}$.
\end{proof}


==> proof-higman.tex <==
\begin{proof}
  We prove that every ideal is a product by introducing a class of finite state automata encoding languages included in $S^*$. More formaly, an $S$-automaton is a tuple $A=(Q,Q_0,F,\Delta)$ where $Q$ is a non-empty finite set of control states, $Q_0\subseteq Q$ is a finite set of initial states, $F\subseteq Q$ is a finite set of final states, and $\Delta\subseteq Q\times (S\cup\{\varepsilon\})\times Q$ is a finite or an infinite set of transitions. A word $\sigma\in S^*$ is said to be accepted by $A$ if there exists an alternating sequence $q_0,\sigma_1,q_1\ldots,\sigma_k,q_k$ with $q_0,\ldots,q_k\in Q$, $\sigma_1,\ldots,\sigma_k\in S\cup\{\varepsilon\}$ such that $q_0\in Q_0$, $q_k\in F$, $\sigma=\sigma_1\ldots\sigma_k$ and such that $(q_{j-1},\varepsilon,q_j)\in\Delta$ for every $1\leq j\leq k$. The set of words accepted by an $S$-automaton is called the language recognizes by the $S$-automaton. A language $L\subseteq S^*$ is said to be $S$-regular if it is recognizable by an $S$-automaton. Classical automata operations can be extended to $S$-automata in such a way that the class of $S$-regular languages is shown to be stable by union, intersection and complement.

  Now, let us consider a downward closed language $L$ of $S^*$. The complement $U=S^*\moins L$ is upward closed. Hence, there exists a finite set $X\subseteq U$ such that $U=\uparrow_{\preceq^*}X$. Observe that for every $x=x_1\ldots x_k$ with $x_j\in S$, the language $\uparrow_{\preceq^*}x$ is equal to $S^*(\uparrow_{\preceq}x_1)S^*\ldots (\uparrow_{\preceq}x_k)S^*$. Such a language is $S$-regular since it is recognized by an $S$-automaton with $k$ control states. Hence $U$ is $S$-regular, and its complement $L$ is also $S$-regular. Now, let $A=(Q,Q_0,F,\Delta)$ be an $S$-automaton recognizing $L$. Since $L$ is downward closed, for every transition $(p,s,q)\in\Delta$ we can add to $\Delta$ transitions $(p,\varepsilon,q)$ and $(p,t,q)$ for every $t\preceq s$ without changing the recognized language. In particular for every $p,q\in Q$, we can assume that the set $\{x\in S\cup\{\varepsilon\} \mid (p,x,q)\in\Delta\}$ is either empty or a set of the form $D\cup\{\varepsilon\}$ where $D$ is a downward closed set of $(S,\preceq)$. Let us consider a strongly connected component of this automaton and let $D$ be the set of $s\in S$ such that the exists a transition $(p,s,q)\in\Delta$ with $p,q$ in the strongly connetced component. Since we can move from one state to any other state of the strongly connected component with $\varepsilon$ transitions, we deduce that the language recognized by this strongly connected component is $D^*$. Since $D$ is downward closed, by decomposing the $S$-automaton $A$ into strongly connected components, we deduce that $L$ is a finite union of languages of the form $L_1\ldots L_k$ where for every $j$, the language $L_j$ is either $D_j^*$ or the language $P_j\cup\{\varepsilon\}$ where $D_j,P_j$ are downward closed sets of $(S,\preceq)$. Lemma~\ref{lem:idealdecomposition} shows that every downward closed set is a finite union of ideals. By decomposing the sets $P_j$, we deduce that $L$ is a finite union of products.

  Now, let $L$ be an ideal of $S^*$. We have proved that it is included into a finite union of products. From Lemma~\ref{lem:insecable}, we deduce that it is included into one of them. In particular it is equal to it Thus every ideal is a product.
\end{proof}
%
